The three-loop unpolarized and polarized non-singlet anomalous dimensions from off shell operator matrix elements

We calculate the unpolarized and polarized three--loop anomalous dimensions and splitting functions $P_{\rm NS}^+, P_{\rm NS}^-$ and $P_{\rm NS}^{\rm s}$ in QCD in the $\overline{\sf MS}$ scheme by using the traditional method of space--like off shell massless operator matrix elements. This is a gauge--dependent framework. For the first time we also calculate the three--loop anomalous dimensions $P_{\rm NS}^{\rm \pm tr}$ for transversity directly. We compare our results to the literature.

==> x20 <==
%--------------------------------------------------------------------------------------------------------
\begin{eqnarray}
%P_{\rm NS}^{(2),s}(z)  &=& - \textcolor{blue}{N_F \frac{d_{abc} d_{abc}}{N_C} }
PNS2s &=& NF dabcdabc
\Biggl\{
-\frac{400}{3} (1-z)
+\Biggl(
        -\frac{2}{3} (100+9 z)
        +\frac{4 (1+z) \big(
                4-7 z+4 z^2\big)}{3 z} \HA_{-1}^2
\nonumber\\ && 
        +\frac{52}{3} (1+z) \HA_{-1}
        +16 \zeta_3
\Biggr) \HA_0
+\Biggl(
        \frac{1}{3} (-38-29 z)
        -\frac{2 (1+z) \big(
                8-5 z+8 z^2\big)}{3 z} \HA_{-1}
\Biggr) \HA_0^2
\nonumber\\ && 
+\frac{2}{9} \big(
        3+8 z^2\big) \HA_0^3
-\frac{1}{3} \HA_0^4
+\Biggl(
        \frac{182}{3} (-1+z)
        +3 (1-z) \HA_0^2
\Biggr) \HA_1
+\Biggl(
        -\frac{82}{3} (1+z)
\nonumber\\ &&         
-6 (1-z) \HA_0
        +2 (1+z) \HA_0^2
        -\frac{16 (1+z) \big(
                2+z+2 z^2\big)}{3 z} \HA_{-1}
\Biggr) \HA_{0,1}
+\Biggl(
        -\frac{52}{3} (1+z)
\nonumber\\ &&         
+\frac{16 \big(
                2+3 z^2\big)}{3 z} \HA_0
        +4 (1-z) \HA_0^2
        -\frac{8 (1+z) \big(
                4-7 z+4 z^2\big)}{3 z} \HA_{-1}
\Biggr) \HA_{0,-1}
+8 (1-z) 
\nonumber\\ && 
\times
\HA_{0,-1}^2
+\Biggl(
        \frac{4}{3} \big(
                3+9 z+8 z^2\big)
        -8 (1+z) \HA_0
\Biggr) \HA_{0,0,1}
+\Biggl(
        \frac{4 \big(
                -8+3 z-21 z^2+8 z^3\big)}{3 z}
\nonumber\\ && 
        -8 (1-z) \HA_0
\Biggr) \HA_{0,0,-1}
+\frac{16 (1+z) \big(
        2+z+2 z^2\big)}{3 z} [\HA_{0,1,-1} + \HA_{0,-1,1}]
\nonumber\\ && 
+\Biggl(
        \frac{8 (1+z) \big(
                4-7 z+4 z^2\big)}{3 z}
        -16 (1-z) \HA_0
\Biggr) \HA_{0,-1,-1}
+\Biggl(
        \frac{2}{3} (67+41 z)
\nonumber\\ &&         
-\frac{2}{3} \big(
                3+27 z+32 z^2\big) \HA_0
        +2 (5+3 z) \HA_0^2
        -\frac{4 (-1+z) \big(
                4+7 z+4 z^2\big)}{3 z} \HA_1
\nonumber\\ &&         
+\frac{4 (1+z) \big(
                4-z+4 z^2\big)}{z} \HA_{-1}
        +8 (1+z) \HA_{0,1}
        -8 (1-z) \HA_{0,-1}
\Biggr) \zeta_2
-2 (3+5 z) \zeta_2^2
\nonumber\\ &&
-\frac{16}{3} \big(
        3+5 z^2\big) \zeta_3
\Biggr\}. 
%\surd
\end{eqnarray}

